Coherence Modeling of Asynchronous Conversations: A Neural Entity Grid Approach

We propose a novel coherence model for written asynchronous conversations (e.g., forums, emails), and show its applications in coherence assessment and thread reconstruction tasks. We conduct our research in two steps. First, we propose improvements to the recently proposed neural entity grid model by lexicalizing its entity transitions. Then, we extend the model to asynchronous conversations by incorporating the underlying conversational structure in the entity grid representation and feature computation. Our model achieves state of the art results on standard coherence assessment tasks in monologue and conversations outperforming existing models. We also demonstrate its effectiveness in reconstructing thread structures.

==> Egrids-background.tex <==
\newcite{Barzilay:2005,Barzilay:2008} introduced an entity-based model for representing and assessing text coherence. Their model represents a text by a two-dimensional array called \textbf{entity grid} that captures transitions of discourse entities across sentences. As shown in Figure \ref{table:doc}, the rows of the grid correspond to sentences, and the columns correspond to discourse entities appearing in the text. They consider noun phrases (NP) as {entities}, and employ a coreference resolver to detect mentions of the same entity (\eg\ \emph{Obama} and \emph{the president}). Each entry $G_{i,j}$ in the entity grid represents the syntactic role that entity $e_j$ plays in sentence $s_i$, which can be one of: subject (\textbf{S}), object (\textbf{O}), or other (\textbf{X}); entities not appearing in a sentence are marked by a special symbol (\textbf{--}). Consider for example the column  for the entity \emph{Eaton} in Figure \ref{table:doc}, [\textsc{X - - S}]. It indicates that Eaton plays an `other' and a `subject' role in the first and the last sentences, respectively, and it is absent from the rest of the sentences. If an entity appears more than once with different grammatical roles in the same sentence, the role with the highest rank (S $\succ$ O $\succ$ X) is considered. 

Motivated by Centering Theory \cite{Grosz:1995}, \newcite{Barzilay:2008} consider \textbf{local entity transitions} as the deciding patterns for text coherence. A {local entity transition} of length $k$ is a sequence of $\{$S,O,X,--$\}^k$ representing grammatical roles played by an entity in $k$ consecutive sentences. Each grid is represented by a vector of $4^k$ transition probabilities computed from the grid. For example, the probability of the transition $[X--]$ in Figure~\ref{table:grid} is $0.079$, computed as a ratio of its frequency (i.e., 3) divided by the total number of transitions of length three (i.e., 38) in the entity grid. 

To distinguish between transitions of important entities from  unimportant ones, \cite{Barzilay:2008} consider the \emph{salience} of the entities, which they quantify by their occurrence frequency in the document. With the feature vector representation, they formulate coherence assessment as a ranking problem in an SVM preference ranking framework \cite{Joachims:2002}. In their experiments, they showed significant improvements in two out of three evaluation tasks when a coreference resolver is used to identify coreferent entities in a text.

   

Subsequent studies proposed to extend the basic entity grid model. \cite{Filippova:2007} attempted to improve the model by grouping entities based on semantic relatedness, but did not get significant improvement. \newcite{Elsner:2008} proposed a \textbf{discourse-new} model and a \textbf{pronoun} model for measuring text coherence. For each mention of referring expressions (\ie\ NPs) in a text, the discourse-new model identifies whether it is the first mention (\emph{discourse-new}) or a subsequent (\emph{discourse-old}) one. Given a text, they run a maximum-entropy classifier to detect each NP as $L_{np} \in \{$\emph{discourse-new, discourse-old}$\}$. The coherence score of the document is then  estimated by  $\prod_{np:NPs}P(L_{np}|np)$. The pronoun model on the other hand uses the joint probability of a pronominal reference $R$ and a referent antecedent $A$ given the Hobbs distance between $R$ and $A$, the number of previous references to $A$, and the number and gender agreements between $R$ and $A$. They show significant improvements by combining the scores of the two coreference inspired models with the score of the basic entity grid model.  


%by taking into account mentions of all referring expression (\ie\ NPs) whether they are first mention (\emph{discourse-new}) or subsequent (\emph{discourse-old}) mentions. Given a document, they run a maximum-entropy classifier to detect each NP as a label $L_{np} \in \{new,old\}$. The coherence score of the document is then  estimated by  $\prod_{np:NPs}P(L_{np}|np)$. 

%In this work, they also estimate text coherence through pronoun coreference modeling.


\newcite{Elsner:2011} proposed a number of improvements. Initially, they show significant improvement by including non-head nouns (\ie\ nouns that do not head NPs) as entities with role `{X}' in the grid. Instead of using a coreference resolver, they match the nouns to detect coreferent entities. By doing so, they not only provide more information to the standard grid, but also maximize coreference recall \cite{Elsner:2010:SHC}. They show further improvements by extending the grid to distinguish between entities of different types by incorporating entity-specific features like named entity, noun class, modifiers, etc.\footnote{Recall that the original entity grid uses only one entity-specific feature, which is \emph{Salience}.} These extensions led to the best results reported so far.

\newcite{Feng:2012} used the basic entity grid representation, but improved its learning to rank scheme. Their model learns not only from original document and its permutations but also from ranking preferences among the permutations themselves. 


\red{Neural Entity Grid} 



==> figures/egrid-tree.tex <==
\begin{table*}[t]
\label{table:tree-grid}
\centering
\resizebox{0.90\linewidth}{!}{
\begin{tabular}{cccc|cccccccccccccccc}
 \multicolumn{3}{c}{Tree structure} & depth& {\rotatebox{90}{CLEANER}} & {\rotatebox{90}{REGEDIT}} & {\rotatebox{90}{TROUBLES}} & {\rotatebox{90}{SYSTEM}} & {\rotatebox{90}{JUNKS}} & {\rotatebox{90}{APPS}} & {\rotatebox{90}{REGISTRY}} & {\rotatebox{90}{BUNCH}} \\ %& {\rotatebox{90}{TERM}} & {\rotatebox{90}{CONCERN}}& {\rotatebox{90}{AEROSPACE}} & {\rotatebox{90}{EMPLOYEES}} & {\rotatebox{90}{SERVICES}} & {\rotatebox{90}{LOS ANGELES}} \\
\toprule
 \multicolumn{3}{c}{ $s_{0}$} & 0 & $-$ & $-$ & $-$ &O& X & X & O & O \\ %&$-$&$-$&$-$&X&$-$&$-$ \\
\multicolumn{3}{c}{ $s_{1}$} & 1 & O       &$-$&$-$&$-$&$-$&$-$& O &$-$ \\ %&S&$-$&$-$&$-$&$-$&$-$ \\
$s_{2}$ & $s_{5}$ & $s_{9}$ &  2  & $-$O$-$ &O$--$ &$---$& $---$& X$--$& $---$&$-$O$-$&O$--$ \\ %&$-$&$-$&$-$&O&O&X \\
$s_{3}$ & $s_{6}$ & $s_{10}$ & 3 & $---$   &S$--$ &$---$& $---$& $---$& $---$ &$---$&$---$ \\ %&$-$&O&X&$-$&$-$& $-$ \\ 
$s_{4}$ & $s_{7}$ & $s_{11}$ & 4 & $---$   &$---$ &$---$& $---$& $-$X$-$ & $---$ &$---$&$---$ \\ %&$-$&O&X&$-$&$-$& $-$ \\ 
& $s_{8}$& $s_{12}$ & 5          & $--$    &$--$ &$--$&  $--$& $--$&  $--$  &$--$&$--$ \\%&$-$&O&X&$-$&$-$& $-$ \\ 
& & $s_{13}$ & 6 & $-$    &$-$ &$-$&  $-$& $-$&  $-$  &$-$&$-$ \\%&$-$&O&X&$-$&$-$& $-$ \\ 
& & $s_{14}$ & 7 & X    &O&$-$&  $-$& $-$&  $-$  &$-$&$-$ \\%&$-$&O&X&$-$&$-$& $-$ \\ 
& & $s_{15}$ & 8 & $-$    &$-$ &$-$&  $-$& $-$&  $-$  &$-$&$-$ \\%&$-$&O&X&$-$&$-$& $-$ \\ 
%\bottomrule
\end{tabular}
}
\caption{Entity grid representation of asynchronous conversations. Legend: S stands for subject, O for object, X for a role other than subject or object, and -- means that an entity does not appear (or absent) in the sentence.}
\end{table*}

==> figures/entity-trans-tree-example.tex <==
\begin{figure}
\centering
\resizebox{1.00\textwidth}{!}{
\small{
\setlength{\tabcolsep}{2em}
\begin{tabular}{cc}
\resizebox{0.25\textwidth}{!}{
\LARGE{
\begin{tikzpicture}[>=stealth, thick]

\node (P1) at (0,6.5) [text width=0.8cm] {$p_1$};

\node (A1) at (0,5) [draw, process, text width=0.8cm, minimum height=2.0cm, align=center] 
{O\\
{O}};

\node (P2) at (-2.5,2) [text width=0.8cm] {$p_2$};

\node (A2) at (-2.5,0.35) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{O\\ 
--\\
--};

\node (P3) at (-0.5,2) [text width=0.8cm] {$p_3$};
\node (A3) at (0,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{O\\ 
--\\
--\\
--};

\node (P4) at (3.1,2) [text width=0.8cm] {$p_4$};
\node (A4) at (2.5,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{O\\ 
--\\
--\\
--};

\node (P4) at (3.1,-2.5) [text width=0.8cm] {$p_5$};

\node (A5) at (2.5,-4) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{S\\ 
--\\
--};

\coordinate (x) at (0,4);
\coordinate (y) at (-2.5,1.45);
\coordinate (z) at (2.5,1.45);
\draw[<-] (x) -- (y);
\draw[<-] (x) -- (z);

%\coordinate (z) at (4.5,0);
%\coordinate (k) at (4.5,-7.7);

\draw[<-] (A1) -- (A3);
%\draw[-] (A1) -- (A3);
%\draw[-] (A1) -- (A4);
\draw[<-] (A4) -- (A5);

%\draw[-] (A1) -- (x);
%\draw[->] (E1) -- (D2);

%\draw[->] (C2) -- (k) -- (z) |- (A2);
%\draw[->] (D2) -- (x) -- (y) |- (A2);

\node (t) at (0, -7) {\Large{(a) Role transition for \textbf{`registry'}}};
\end{tikzpicture}}
}


&

\resizebox{0.25\textwidth}{!}{
\LARGE{
\begin{tikzpicture}[>=stealth, thick]


\node (P0) at (-3,6.5) [text width=0.8cm] {{\bf registry}};


\node (P1) at (-1, 5.5) [text width=0.8cm] {$P_2$};
\node (P1) at (-2.5, 5.5) [text width=0.8cm] {$P_1$};
\node (P1) at (-4, 5.5) [text width=0.8cm] {$P_0$};

\node (P1) at (-5.5, 4.5) [text width=0.8cm] {$l_0$};
\node (P1) at (-1, 4.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-2.5, 4.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-4, 4.5) [text width=0.8cm] {{\bf O}};

\node (P1) at (-5.5, 3.5) [text width=0.8cm] {$l_1$};
\node (P1) at (-1, 3.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-2.5, 3.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-4, 3.5) [text width=0.8cm] {{\bf O}};

\node (P1) at (-5.5, 2.5) [text width=0.8cm] {$l_2$};
\node (P1) at (-1, 2.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-2.5, 2.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-4, 2.5) [text width=0.8cm] {{\bf O}};

\node (P1) at (-5.5, 1.5) [text width=0.8cm] {$l_3$};
\node (P1) at (-1, 1.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, 1.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-4, 1.5) [text width=0.8cm] {{\bf --}};

\node (P1) at (-5.5, 0.5) [text width=0.8cm] {$l_4$};
\node (P1) at (-1, 0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, 0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-4, 0.5) [text width=0.8cm] {{\bf --}};

\node (P1) at (-5.5, -0.5) [text width=0.8cm] {$l_5$};
\node (P1) at (-1, -0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, -0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-4, -0.5) [text width=0.8cm] {$\phi$};


\node (P1) at (-5.5, -1.5) [text width=0.8cm] {$l_6$};
\node (P1) at (-1, -1.5) [text width=0.8cm] {{\bf S}};
\node (P1) at (-2.5, -1.5) [text width=0.8cm] {$\phi$};
\node (P1) at (-4, -1.5) [text width=0.8cm] {$\phi$};

\node (P1) at (-5.5, -2.5) [text width=0.8cm] {$l_7$};
\node (P1) at (-1, -2.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, -2.5) [text width=0.8cm] {$\phi$};
\node (P1) at (-4, -2.5) [text width=0.8cm] {$\phi$};

\node (P1) at (-5.5, -3.5) [text width=0.8cm] {$l_8$};
\node (P1) at (-1, -3.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, -3.5) [text width=0.8cm] {$\phi$};
\node (P1) at (-4, -3.5) [text width=0.8cm] {$\phi$};



\coordinate (x3) at (-5, 6.5);
\coordinate (y3) at (-5,-4);
\draw[-] (x3) -- (y3);

\coordinate (x4) at (-6.5,5);
\coordinate (y4) at (0, 5);
\draw[-] (x4) -- (y4);

\coordinate (x5) at (-6.5,-4);
\coordinate (y5) at (0, -4);
\draw[-] (x5) -- (y5);

\node (t) at (0, -6) {\Large{(c) Grid representations}};

\end{tikzpicture}
}
}



\\


\end{tabular}
}
}

\caption{Grammatical role transition for two entities and their corresponding grid representations. Symbol $\phi$ in the grid represents zero-padding to match the maximum depth of a tree.
}
\label{fig:ent-grid-con}
\end{figure}




 
 
 \begin{comment}
 \begin{figure*}
\centering
\resizebox{1.00\textwidth}{!}{
\small{
\setlength{\tabcolsep}{2em}
\begin{tabular}{ccc}
%\resizebox{0.25\textwidth}{!}{
\LARGE{
\begin{tikzpicture}[>=stealth, thick]

\node (P1) at (0,6.5) [text width=0.8cm] {$p_1$};

\node (A1) at (0,5) [draw, process, text width=0.8cm, minimum height=2.0cm, align=center] 
{O\\
{O}};

\node (P2) at (-2.5,2) [text width=0.8cm] {$p_2$};

\node (A2) at (-2.5,0.35) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{O\\ 
--\\
--};

\node (P3) at (-0.5,2) [text width=0.8cm] {$p_3$};
\node (A3) at (0,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{O\\ 
--\\
--\\
--};

\node (P4) at (3.1,2) [text width=0.8cm] {$p_4$};
\node (A4) at (2.5,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{O\\ 
--\\
--\\
--};

\node (P4) at (3.1,-2.5) [text width=0.8cm] {$p_5$};

\node (A5) at (2.5,-4) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{S\\ 
--\\
--};

\coordinate (x) at (0,4);
\coordinate (y) at (-2.5,1.45);
\coordinate (z) at (2.5,1.45);
\draw[<-] (x) -- (y);
\draw[<-] (x) -- (z);

%\coordinate (z) at (4.5,0);
%\coordinate (k) at (4.5,-7.7);

\draw[<-] (A1) -- (A3);
%\draw[-] (A1) -- (A3);
%\draw[-] (A1) -- (A4);
\draw[<-] (A4) -- (A5);

%\draw[-] (A1) -- (x);
%\draw[->] (E1) -- (D2);

%\draw[->] (C2) -- (k) -- (z) |- (A2);
%\draw[->] (D2) -- (x) -- (y) |- (A2);

\node (t) at (0, -7) {\Large{(a) Role transition for \textbf{`registry'}}};
\end{tikzpicture}}
%}
&
%\resizebox{0.5\textwidth}{!}{
\LARGE{
\begin{tikzpicture}[>=stealth, thick]

\node (P1) at (0,6.5) [text width=0.8cm] {$p_1$};

\node (P1) at (0,6.5) [text width=0.8cm] {$p_1$};

\node (A1) at (0,5) [draw, process, text width=0.8cm, minimum height=2.0cm, align=center] 
{X\\
{--}};

\node (P2) at (-2.5,2) [text width=0.8cm] {$p_2$};

\node (A2) at (-2.5,0.35) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{X\\ 
--\\
--};

\node (P3) at (-0.5,2) [text width=0.8cm] {$p_3$};
\node (A3) at (0,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{--\\ 
--\\
X\\
--};

\node (P4) at (3.1,2) [text width=0.8cm] {$p_4$};
\node (A4) at (2.5,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{X\\ 
--\\
--\\
--};

\node (P4) at (3.1,-2.5) [text width=0.8cm] {$p_5$};

\node (A5) at (2.5,-4) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{--\\ 
--\\
--};

\coordinate (x) at (0,4);
\coordinate (y) at (-2.5,1.45);
\coordinate (z) at (2.5,1.45);
\draw[<-] (x) -- (y);
\draw[<-] (x) -- (z);

%\coordinate (z) at (4.5,0);
%\coordinate (k) at (4.5,-7.7);

\draw[<-] (A1) -- (A3);
%\draw[-] (A1) -- (A3);
%\draw[-] (A1) -- (A4);
\draw[<-] (A4) -- (A5);

%\draw[-] (A1) -- (x);
%\draw[->] (E1) -- (D2);

%\draw[->] (C2) -- (k) -- (z) |- (A2);
%\draw[->] (D2) -- (x) -- (y) |- (A2);

%\node (t) at (0, -6) {\Large{(b) Conversational structure}};
\node (t) at (0, -7) {\Large{(b) Role transition for \textbf{`junk'}}};
\end{tikzpicture}
}
%}
&
\LARGE{
\begin{tikzpicture}[>=stealth, thick]


\node (P0) at (-3,6.5) [text width=0.8cm] {{\bf registry}};
\node (P0) at (2, 6.5) [text width=0.8cm] {{\bf junk}};

\node (P1) at (-1, 5.5) [text width=0.8cm] {$P_2$};
\node (P1) at (-2.5, 5.5) [text width=0.8cm] {$P_1$};
\node (P1) at (-4, 5.5) [text width=0.8cm] {$P_0$};
\node (P1) at (1, 5.5) [text width=0.8cm] {$P_0$};
\node (P1) at (2.5, 5.5) [text width=0.8cm] {$P_1$};
\node (P1) at (4, 5.5) [text width=0.8cm] {$P_2$};

\node (P1) at (-5.5, 4.5) [text width=0.8cm] {$l_0$};
\node (P1) at (-1, 4.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-2.5, 4.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-4, 4.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (1, 4.5) [text width=0.8cm] {{\bf X}};
\node (P1) at (2.5, 4.5) [text width=0.8cm] {{\bf X}};
\node (P1) at (4, 4.5) [text width=0.8cm] {{\bf X}};

\node (P1) at (-5.5, 3.5) [text width=0.8cm] {$l_1$};
\node (P1) at (-1, 3.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-2.5, 3.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-4, 3.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (1, 3.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (2.5, 3.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (4, 3.5) [text width=0.8cm] {{\bf --}};

\node (P1) at (-5.5, 2.5) [text width=0.8cm] {$l_2$};
\node (P1) at (-1, 2.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-2.5, 2.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (-4, 2.5) [text width=0.8cm] {{\bf O}};
\node (P1) at (1, 2.5) [text width=0.8cm] {{\bf X}};
\node (P1) at (2.5, 2.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (4, 2.5) [text width=0.8cm] {{\bf X}};

\node (P1) at (-5.5, 1.5) [text width=0.8cm] {$l_3$};
\node (P1) at (-1, 1.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, 1.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-4, 1.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (1, 1.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (2.5, 1.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (4, 1.5) [text width=0.8cm] {{\bf --}};

\node (P1) at (-5.5, 0.5) [text width=0.8cm] {$l_4$};
\node (P1) at (-1, 0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, 0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-4, 0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (1, 0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (2.5, 0.5) [text width=0.8cm] {{\bf X}};
\node (P1) at (4, 0.5) [text width=0.8cm] {{\bf --}};

\node (P1) at (-5.5, -0.5) [text width=0.8cm] {$l_5$};
\node (P1) at (-1, -0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, -0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-4, -0.5) [text width=0.8cm] {$\phi$};
\node (P1) at (1, -0.5) [text width=0.8cm] {{$\phi$}};
\node (P1) at (2.5, -0.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (4, -0.5) [text width=0.8cm] {{\bf --}};


\node (P1) at (-5.5, -1.5) [text width=0.8cm] {$l_6$};
\node (P1) at (-1, -1.5) [text width=0.8cm] {{\bf S}};
\node (P1) at (-2.5, -1.5) [text width=0.8cm] {$\phi$};
\node (P1) at (-4, -1.5) [text width=0.8cm] {$\phi$};
\node (P1) at (1, -1.5) [text width=0.8cm] {$\phi$};
\node (P1) at (2.5, -1.5) [text width=0.8cm] {$\phi$};
\node (P1) at (4, -1.5) [text width=0.8cm] {{\bf --}};

\node (P1) at (-5.5, -2.5) [text width=0.8cm] {$l_7$};
\node (P1) at (-1, -2.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, -2.5) [text width=0.8cm] {$\phi$};
\node (P1) at (-4, -2.5) [text width=0.8cm] {$\phi$};
\node (P1) at (1, -2.5) [text width=0.8cm] {$\phi$};
\node (P1) at (2.5, -2.5) [text width=0.8cm] {$\phi$};
\node (P1) at (4, -2.5) [text width=0.8cm] {{\bf --}};

\node (P1) at (-5.5, -3.5) [text width=0.8cm] {$l_8$};
\node (P1) at (-1, -3.5) [text width=0.8cm] {{\bf --}};
\node (P1) at (-2.5, -3.5) [text width=0.8cm] {$\phi$};
\node (P1) at (-4, -3.5) [text width=0.8cm] {$\phi$};
\node (P1) at (1, -3.5) [text width=0.8cm] {$\phi$};
\node (P1) at (2.5, -3.5) [text width=0.8cm] {$\phi$};
\node (P1) at (4, -3.5) [text width=0.8cm] {{\bf --}};

\coordinate (x1) at (-0.05,6.5);
\coordinate (y1) at (-0.05,-4);
\coordinate (x2) at (0.05,6.5);
\coordinate (y2) at (0.05,-4);

\draw[-] (x1) -- (y1);
\draw[-] (x2) -- (y2);


\coordinate (x3) at (-5, 6.5);
\coordinate (y3) at (-5,-4);
\draw[-] (x3) -- (y3);

\coordinate (x4) at (-6.5,5);
\coordinate (y4) at (5, 5);
\draw[-] (x4) -- (y4);

\coordinate (x5) at (-6.5,-4);
\coordinate (y5) at (5, -4);
\draw[-] (x5) -- (y5);

\node (t) at (0, -6) {\Large{(c) Grid representations}};

\end{tikzpicture}
}
%}



\\


\end{tabular}
}
}

\caption{Grammatical role transition for two entities and their corresponding grid representations. Symbol $\phi$ in the grid represents zero-padding to match the maximum depth of a tree.
}
\label{fig:ent-grid-con}
\end{figure*}









%===========================================


%\resizebox{0.25\columnwidth}{!}{
%\node (P1) at (0,6.5) [text width=0.8cm] {$p_1$};
\LARGE{
\begin{tabular}{l|ccc||ccc}
& \multicolumn{3}{c}{\textbf{registry}} & \multicolumn{3}{c}{\textbf{junk}}\\
& $P_0$ & $P_1$ & $P_2$ & $P_0$ & $P_1$ & $P_2$ \\
\hline
$l_0$ & O  & O & O & X  & X & X \\ 
$l_1$ & O  & O & O & --  & -- & --\\
$l_2$ & O  & O & O & X  & -- & X \\
$l_3$ & -- & -- & -- & -- & -- & --  \\
$l_4$ & -- & -- & --  & -- & X & -- \\
$l_5$ & $\phi$ & -- & -- & $\phi$ & --& --\\ 
$l_6$ & $\phi$ & $\phi$ & S & $\phi$ & $\phi$ & -- \\ 
$l_7$ & $\phi$ & $\phi$ & -- & $\phi$ & $\phi$ & -- \\ 
$l_8$ & $\phi$ & $\phi$ & -- & $\phi$ & $\phi$ & -- \\ 
\bottomrule 
\end{tabular}
}

&
\LARGE{
\begin{tikzpicture}[>=stealth, thick]

\node (P1) at (0,6.5) [text width=0.8cm] {$p_1$};

\node (A1) at (0,5) [draw, process, text width=0.8cm, minimum height=2.0cm, align=center] 
{X\\
{--}};

\node (P2) at (-2.5,2) [text width=0.8cm] {$p_2$};

\node (A2) at (-2.5,0.35) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{X\\ 
--\\
--};

\node (P3) at (-0.5,2) [text width=0.8cm] {$p_3$};
\node (A3) at (0,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{--\\ 
--\\
X\\
--};

\node (P4) at (3.1,2) [text width=0.8cm] {$p_4$};
\node (A4) at (2.5,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{X\\ 
--\\
--\\
--};

\node (P4) at (3.1,-2.5) [text width=0.8cm] {$p_5$};

\node (A5) at (2.5,-4) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{--\\ 
--\\
--};

\coordinate (x) at (0,4);
\coordinate (y) at (-2.5,1.45);
\coordinate (z) at (2.5,1.45);
\draw[<-] (x) -- (y);
\draw[<-] (x) -- (z);

%\coordinate (z) at (4.5,0);
%\coordinate (k) at (4.5,-7.7);

\draw[<-] (A1) -- (A3);
%\draw[-] (A1) -- (A3);
%\draw[-] (A1) -- (A4);
\draw[<-] (A4) -- (A5);

%\draw[-] (A1) -- (x);
%\draw[->] (E1) -- (D2);

%\draw[->] (C2) -- (k) -- (z) |- (A2);
%\draw[->] (D2) -- (x) -- (y) |- (A2);

%\node (t) at (0, -6) {\Large{(b) Conversational structure}};
\node (t) at (0, -6) {\Large{(b) Grammatical role transition for \textbf{`junk'}}};

\end{tikzpicture}
}
\end{comment}


==> figures/thread-tree-example.tex <==
\begin{figure*}
\centering
\resizebox{0.90\linewidth}{!}{
\small{
\setlength{\tabcolsep}{4em}
\begin{tabular}{cc}
\begin{tikzpicture}[>=stealth, thick]

\node (A1) at (0,1.19) [draw, process, text width=10.5cm, minimum height=0.5cm, align=center] 
{\textbf{Author:} barspinboy \textbf{ Post ID:} 1};

\node (A2) at (0,0) [draw, process, text width=10.5cm, minimum height=0.7cm, align=left] 
{ \textbf{$s_0$:} im having troubles since i uninstall some of my apps, then when i checked my system registry bunch of junks were left behind by the apps i already uninstall.\\ 
$s_1$: is there any way i could clean my registry aside from expensive registry cleaners. };
%my computer suffers from crash and slow start up. please give me advice so i can clear up ...};

\node (B1) at (0,-2.0) [draw, process, text width=10.5cm, minimum height=0.5cm, align=center] 
{\textbf{Author:} kees bakker \textbf{ Post ID:} 2};

\node (B2) at (0,-2.83) [draw, process, text width=10.5cm, minimum height=0.7cm, align=left] 
{
$s_2$: use regedit to delete the `bunch of junks' you found {in registry}.\\ 
$s_3$: regedit is free, but depending on which applications it were .. \\
$s_4$: it's somewhat doubtful there will be less crashes and faster setup.};

\node (C1) at (0,-4.5) [draw, process, text width=10.5cm, minimum height=0.5cm, align=center] 
{\textbf{Author:} willy \textbf{ Post ID:} 3};

\node (C2) at (0,-5.72) [draw, process, text width=10.5cm, minimum height=0.7cm, align=left] 
{$s_5$: i tend to use ccleaner (google for it) as a registry (and system) cleaner. \\ 
$s_6$: using its defaults does pretty well.  \\
$s_7$: in no way will it cure any hardcore problems as you mentioned, ``crashes'', but it should clean some of the junk out.  \\
$s_8$: i further suggest, .. };

\node (D1) at (0,-8.0) [draw, process, text width=10.5cm, minimum height=0.5cm, align=center] 
{\textbf{Author:} caktus \textbf{ Post ID:} 4};

\node (D2) at (0,-9.0) [draw, process, text width=10.5cm, minimum height=0.7cm, align=left] 
{ $s_{9}$: try regseeker {to clean your registry junk}. \\ 
$s_{10}$: it's free and pretty safe to use automatic.  \\
$s_{11}$: then clean out temp files (don't compress any files or use indexing.)  \\
$s_{12}$: if the c drive is compressed, then uncompress it.};

\node (E1) at (0,-11.0) [draw, process, text width=10.5cm, minimum height=0.5cm, align=center] 
{\textbf{Author:} barspinboy \textbf{ Post ID:} 5 };

\node (E2) at (0,-12.0) [draw, process, text width=10.5cm, minimum height=0.7cm, align=left ] 
{$s_{13}$: thanks guyz, {my registry is clean now} \\
$s_{14}$: i tried all those suggestions you mentioned ccleaners regedit defragmentation and uninstalling process. \\
$s_{15}$: it all worked out and i suffer no more from crashes and ..};

\coordinate (x) at (-6.0,-9);
\coordinate (y) at (-6.0,0);

\coordinate (z) at (6.0,0.0);
\coordinate (k) at (6.0,-5.8);

\draw[->] (B1) -- (A2);
\draw[->] (E1) -- (D2);

\draw[->] (C2) -- (k) -- (z) |- (A2);
\draw[->] (D2) -- (x) -- (y) |- (A2);

\node (t) at (0, -14) {\Large{(a) A forum conversation}};

\end{tikzpicture} 

&
\LARGE{
\begin{tikzpicture}[>=stealth, thick]

\node (P1) at (0,6.5) [text width=0.8cm] {$p_1$};

\node (A1) at (0,5) [draw, process, text width=0.8cm, minimum height=2.0cm, align=center] 
{$s_0$\\
{$s_1$}};

\node (P2) at (-2.5,2) [text width=0.8cm] {$p_2$};

\node (A2) at (-2.5,0.35) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{$s_2$\\ 
$s_3$\\
$s_4$};

\node (P3) at (-0.5,2) [text width=0.8cm] {$p_3$};
\node (A3) at (0,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{$s_5$\\ 
$s_6$\\
$s_7$\\
$s_8$};

\node (P4) at (3.1,2) [text width=0.8cm] {$p_4$};
\node (A4) at (2.5,0) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{$s_9$\\ 
$s_{10}$\\
$s_{11}$\\
$s_{12}$};

\node (P4) at (3.1,-2.5) [text width=0.8cm] {$p_5$};

\node (A5) at (2.5,-4) [draw, process, text width=0.8cm, minimum height=0.5cm, align=center] 
{$s_{13}$\\ 
$s_{14}$\\
$s_{15}$};

\coordinate (x) at (0,4);
\coordinate (y) at (-2.5,1.45);
\coordinate (z) at (2.5,1.45);
\draw[<-] (x) -- (y);
\draw[<-] (x) -- (z);

%\coordinate (z) at (4.5,0);
%\coordinate (k) at (4.5,-7.7);

\draw[<-] (A1) -- (A3);
%\draw[-] (A1) -- (A3);
%\draw[-] (A1) -- (A4);
\draw[<-] (A4) -- (A5);

%\draw[-] (A1) -- (x);
%\draw[->] (E1) -- (D2);

%\draw[->] (C2) -- (k) -- (z) |- (A2);
%\draw[->] (D2) -- (x) -- (y) |- (A2);

\node (t) at (0, -6) {\Large{(b) Conversational structure}};

\end{tikzpicture}
}


\end{tabular}
}
}
\vspace{-0.5em}
\caption{(a) A forum conversation, and (b) the thread structure of the conversation using `reply-to' links; $p_k$ denotes post with id $k$, and $s_i$ denotes $i$-th sentence in the temporal order of the conversation.}
\label{fig:thread-tree}
\end{figure*}
